HiRace: Accurate and Fast Source-Level Race Checking of GPU Programs

Data races are egregious parallel programming bugs on CPUs. They are even worse on GPUs due to the hierarchical thread and memory structure, which makes it possible to write code that is correctly synchronized within a thread group while not being correct across groups. Thus far, all major data-race checkers for GPUs suffer from at least one of the following problems: they do not check races in global memory, do not work on recent GPUs, scale poorly, have not been extensively tested, miss simple data races, or are not dependable without detailed knowledge of the compiler. Our new data-race detection tool, HiRace, overcomes these limitations. Its key novelty is an innovative parallel finite-state machine that condenses an arbitrarily long access history into a constant-length state, thus allowing it to handle large and long-running programs. HiRace is a dynamic tool that checks for thread-group shared memory and global device memory races. It utilizes source-code instrumentation, thus avoiding driver, compiler, and hardware dependencies. We evaluate it on a modern calibrated data-race benchmark suite. On the 580 tested CUDA kernels, 346 of which contain data races, HiRace finds races missed by other tools without false alarms and is more than 10 times faster on average than the current state of the art, while incurring only half the memory overhead.

==> figures/code_litmus_subwarp.tex <==
\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={subwarp litmus test},label={lst:litmus-sw}]
__global__
void race_warpsync(int* data, int len) {
    int tid = threadIdx.x + blockIdx.x * blockDim.x;
    unsigned two_thread_mask = 0xc0000000;
    
    if ( tid < len-1 ) {
        if (tid < 16) {
            data[tid+1] = 0;
        }
        __syncwarp(two_thread_mask);
        data[tid] = 1; // race!
    }
}
\end{lstlisting}
\end{minipage}

==> figures/code_litmus_threadfence.tex <==
\begin{minipage}{\linewidth}
\begin{lstlisting}[caption={threadfence litmus test},label={lst:litmus-fence}]
__global__
void race_tfence(int* data, int len) {
    int tid = threadIdx.x + blockIdx.x * blockDim.x;
    if ( tid < len-1 ) {
        data[tid] = tid;
        __threadfence();
        data[tid+1] += tid; // race!
    }
}
\end{lstlisting}
\end{minipage}

==> figures/code_wwrace_nosync.tex <==
\begin{minipage}{\linewidth}\begin{lstlisting}[caption=write-write data race,label={lst:ww-nosync}]
__global__
void race_simple(int* data) {
    int tid = threadIdx.x;

    data[0] = tid; \\ race!
    
}
\end{lstlisting}
\end{minipage}

==> figures/litmus_finiteHistory.tex <==
\begin{minipage}{0.95\linewidth}
\begin{listing}
    \begin{minted}{c}
        int main() {
          printf("hello, world");
          return 0;
        }
    \end{minted}
    \caption{finite history litmus test}
    \label{lst:litmus-finiteHistory}
\end{listing}
\end{minipage}
% __global__ void litmus_multiRead_Race(int* data, int len)
% {
%   unsigned tid = threadIdx.x + blockIdx.x * blockDim.x;
%   int local_sum = 0;
  
%   if (tid < len-1) {
%     local_sum = data[tid]; // history lost
%     local_sum += data[tid+1];
    
%     data[tid+1]=local_sum; // race!
%   }
% }

==> sections/design-gg.tex <==


We now describe the design of \hirace via the   simple CUDA-like program (Listing~\ref{ex1-ill}, Example 1), by describing the state-machine actions for one arbitrary memory location (all other locations have a similar associated state machine).
%
Just for the sake of illustration, we consider running this code 
with eight threads, two threads per
warp,  two warps per thread block, 
and two thread blocks
(Figure~\ref{ex1-grid}).
%
We will focus on the thread shown in red with a thread ID (TID) of $3$ (counting from the leftmost thread).


%---
\begin{minipage}{\linewidth}\begin{lstlisting}[caption={Illustrative Example 1},label={ex1-ill}, basicstyle=\small]
kernel(int* data) {
  tid = threadIdx.x;
  bid = blockIdx.x;
  tmp = data[0];
  // __syncthreads();
  data[0] = tid + tmp;
}
\end{lstlisting}
\end{minipage}

\begin{figure}[h]
\includegraphics[scale=.3]{figures/illustration-state-trans.png}
\caption{Grid of CUDA threads assumed in Example-1}
\label{ex1-grid}
\end{figure}

 
\hirace employs a shadow memory structure 
for each data location
(Figure~\ref{fig:ssm_shadow}).
%
Thus, each array element \texttt{data[i]}
has an associated shadow structure
\texttt{shadow[i]} whose fields record the thread ID 
of the last accessing thread for that location.
%
Initially, all the \texttt{State} entries begin at state \texttt{INIT}
(full state-machines presented later).
%
The \texttt{Block AP ID} is the number of barriers seen by a thread.\footnotemark
%
\footnotetext{Here, ``AP'' stands for ``asynchronous parallel region'' (the instructions
executed by all the threads between
successive barrier encounters within
 a thread block). We borrow this term
 from~\cite{LD-race-checker}.}
%


\input{sections/instrumentation.tex}


 

Whenver 
\texttt{data[i]}
is accessed, the \texttt{Block AP ID}
and \texttt{Thread ID} of the accessing thread 
is recorded into
\texttt{shadow[i]}, and \texttt{State} is advanced
as defined
in Table~\ref{tab:illustrative-table}.
%
For example, after Line 4 is executed by the thread with TID 3 (the red thread), 
the Block ID is set to 0, the Thread ID field is set to 3 and the state is updated to \texttt{Read}
(Entry 1 in the table).
%
Subsequently, we will assume that TID 4 also reads this line, creating Entry 2 of the table.
%
The state recorded is \texttt{TID} of 4,
and \texttt{State} remains at \texttt{Read}, meaning the synchronization scope at which this line was read has not changed (Entry Number 2).

Now, assume that TID 0 reads the same location; since this is a thread outside of the warp but within the same thread block, the line is advanced to the \texttt{BRead} state (Entry 3).
%
This indicates  that any subsequent
write within the same block must be separated by a Barrier (none in this example).
%
At this point, suppose TID 5 reads the same
location at line 4.
%
This creates Entry 4, which puts the line in state \texttt{GRead}.
%
All subsequent reads in this program at Line 4
will keep this line in \texttt{GRead}
which is the {\em least permissive read state}
in the sense that {\em any write to this location
} will be flagged as a Race---what Entry 5a shows, when Thread 2 executes Line 6.

Alternatively, let us uncomment the
\texttt{syncthreads()} and run forward from Entry 4 to create Entry 5b.
%



\input{sections/example-transitions.tex}

   
Figure~\ref{fig:ssm_nosync} summarizes these in a single state machine that covers cases with no barriers.
%
Figure~\ref{fig:ssm_bsync} is the 
state machine with details added to depict the effect of barriers.
%
In the previous racing example, if  a barrier is placed before the last line (the write), then
when that barrier is encountered, there will be a transition to XXX and then when the write is encountered, there is a transition to YYY.
%
The key takeaways of \hirace's design are as follows:
%
\begin{compactitem}
    \item Only the last writer is tracked
    \item There are natural invariants at each level (mention a few)

    \item If atomics are included, these changes happen

    \item If warp-sync happens, these changes happen.
\end{compactitem}

==> sections/future-work.tex <==
Possible directions:

\begin{itemize}
    \item efficient support for locks
    \item formal verification (proofs)
    \item performance study to understand tradeoff / limitations of state machine encoding
    \item automate instrumentation (stick with source? or just IR level?)
    \item extend to fully heterogeneous systems (cover unified memory, cover both host and dev. memory with one interface)
    \item extend to other devices (AMD, intel... more generic, like fpga? dunno)
    \item add static analysis pass, either static pass to aid dynamic impl., or standalone static, or both eventually
    \item generalizing algorithm to be customized through user configuration (i.e. Kokkos-inspired user definition of memory/execution structure.) basically, automatically determine both (1) internal state machine structure to handle specified layers of hierarchy, instead of having it designed to fit current CUDA design, and also (2) determine trade-off point for performance in various systems and implement automatic switching or application of multiple methods... for example, TSan method might work better up to maybe 16 or 32 threads with arbitrary interleaving / sync groupings, so we could instr. tsan for that code, but still use our state safety method for other code segments (like other devices in system, or sections with more abstract threads defined for an OMP region for example)
\end{itemize}

==> sections/misc.tex <==
\begin{itemize}
    \item \textbf{TODO: Sanitize for double-blind review!}
    \item Supercomputing info: \url{https://sc23.supercomputing.org/program/papers/}
    \item Submission deadline: Abstract 03/30, full 04/06
    \item Maximum 10 pages (excl. bib)
    \item reproducibility/artifacts important
\end{itemize}


some meeting notes:
martin paper ideas:
1. first just explain simple state machine (maybe single block with syncthreads.)
2. now explain in text only how to extend to support multi block, then others, etc.
3. then describe verification with model checker
4. maybe demo this process against the simple model (like show a simple murphi model tested against the simpler state machine.)
5. then jsut say full model will be released with code.

main thing is to translate the key idea.

one approach is to tackle the problems reviewers might have with verification specifically... i.e. can we prove explicitly that the data we track is enough.

be sure to explicitly state all verified assertions / properties

martins paper writing :

1. outline
2. intro
3. then explain approach in detail
4. related works
5. methodology / exper.
6. results
7. then abstract / conclusions

paper is not a description of your research, but teaching people how to repeat what you did

==> sections/related-work.tex <==
\iguard (and predecessor \scord) is the main comparison, though largely discussed in evaluation... Of course the older tools are relevant (\barracuda, \pug, \curd, \ld.)

potential issues to test in \iguard:
\begin{itemize}
    \item threadfence: just compares counters, but threadfence doesn't synchronize. so, does it miss races when threadfence is used as if it were syncthreads?
    \item warp-sync stuff: checks activemask for determining active threads, but this isn't supported by current cuda semantics, so can we get this to fail?
    \item compares against last accessor and last writer only, probably easy to break this, and our tool should catch.
\end{itemize}

threadsanitizer is also quite related in that, as far as i know, it's probably the "baseline" for practical race detection in a general sense. It of course doesn't apply to CUDA directly, but worth discussing briefly the expected difference in memory overhead and thread communication for their method against ours when run on gpu. main comparison for tsan design will prob. be in background.
